Joint learning of images and videos with a single Vision Transformer

In this study, we propose a method for jointly learning of images and videos using a single model. In general, images and videos are often trained by separate models. We propose in this paper a method that takes a batch of images as input to Vision Transformer IV-ViT, and also a set of video frames with temporal aggregation by late fusion. Experimental results on two image datasets and two action recognition datasets are presented.

==> main_text.tex <==



\section{はじめに}

% 本稿では，単一モデルを用いたマルチドメインなデータの学習方法を提案する．

近年，深層学習の発展に伴い，様々なタスクが研究されている．
その中でも，画像認識と動画認識の研究は盛んに行われている．
画像認識は古くから取り組まれているタスクであり，
数多くの深層学習モデルが提案されている\cite{Dosovitskiy_2021_ViT,He_2016_CVPR, Alex_NeurIPS2012_AlexNet,Simonyan_arXiv2014_VGG,Szegedy_arXiv2014_GoogLeNet}．
またそのためのデータセットも数多く公開されている\cite{Deng_IEEE2009_ImageNet, Lecun_IEEE1998_MNIST}．
動画認識の研究も長い歴史があり\cite{Kensho_IMP2020_video_recog_3D_conv, Yu_2022_human_action_recog,Zhu_arXiv2020_comprehensive}，
大規模なデータセット
\cite{Kuehne_ICCV2011_HMDB51, Li_arXiv2020_AVA-Kinetics,Soomro_arXiv2012_UCF101}
と様々なモデル
\cite{Arnab_ICCV2021_ViVit, Joao_CVPR2017_I3D,Feichtenhofer_CVPR2020_x3d,Feichtenhofer_ICCV2019_SlowFast,Hara_CVPR2018_3DResNet,Karen_NeurIPS2014_TwoStream,Du_ICCV2015_C3D,Zhang_ACMMM2021_TokenShift}
が提案されている．
この画像や動画像のような，扱うデータの種類のことをモード（mode）と呼び，
複数のモードを扱う手法をマルチモーダル（multi-modal）やクロスモーダル（cross-modal）と呼ぶ．
メジャーなモードは，画像や動画像の他にも，自然言語や音声がある．
深層学習以前と比較して，言語や音声と画像・動画像を同時に学習する
マルチモーダルな手法の研究は比較的容易になっており，
画像・動画像とテキストを扱う手法\cite{Aafaq_arXiv2018_Video_captioning_survey, Stefanini_arXiv2021_Video_Caption}や，
画像・動画像と音声を扱う手法\cite{Zhang_CVPR2022, Zhu_arXiv2020_Audio_survey}，
動画像と音声を扱う手法\cite{Jaegle_ICML2021_Perceiver}など，
マルチモーダルな研究は多数存在する．


画像と動画像は，言語や音声と比較して，類似したモードとみなされることが多く，
画像と動画像を同時に扱うようなマルチモーダルな研究はあまり行われて来なかった．
一方で，画像や動画像のそれぞれにおいて
ドメイン適応などの研究は盛んに行われてきた\cite{redko_arXiv2020,wang_Elsevier2018,wilson_arXiv2020}．

ドメインとは，データセット固有の傾向や特徴のことを指し，
通常，モデルはドメインやデータセットが異なると再学習する必要がある．
ドメイン適応は，
異なる2つのドメイン間で同じモデルを使用できるようにする手法の総称である．
またマルチドメイン学習\cite{Li_2019_CVPR,Omi_IEICE-ED2022_MDL,Rebuffi_2018_CVPR}や
マルチデータセット学習\cite{Liang_NeurIPS2022_Multi-Dataset,Zhou_2022_CVPR}は，
異なる複数のドメインのデータに対して単一のモデルを学習する手法である．


近年のVision Transformer（ViT）\cite{Dosovitskiy_2021_ViT}の急速な普及に伴って，
画像と動画像を単一モデルで学習する研究が登場してきた\cite{Fan_2022_SIFAR,Girdhar_CVPR2022_Omnivore,Likhosherstov_arXiv2021_PolyViT,Girdhar_arXiv2022_OmniMAE}．
CNNを用いた画像認識モデルや動画認識モデルは多数提案されているが，そのほとんどは別々に手法が開発されていた．
この理由は，画像と動画像には時間軸という違いが存在するからである．
画像はフレーム数が1枚の動画像とみなせば，1フレーム内に全情報が含まれる．
一方，動画像はフレーム数は2以上であり，各フレームに情報が振り分けられ，
どのフレームに重要な情報が入っているかを考慮し，学習する必要がある．
動画像中のRGB1フレームを利用する動作認識モデルも提案された\cite{Wang_ECCV2016_TSN}が，
時間情報のモデル化が重要であるため，
動画像の認識においては時間情報の取り扱いについて様々な工夫が提案された
\cite{Tran_2018CVPR_R(2+1)D,Wang_2018CVPR_NonLocal}．

この研究の流れにおいては，静止画像を同時に学習することは考慮されてこなかった．
しかしTransformer \cite{Vaswani_arXiv2017_transformer}が普及し，画像認識モデルであるViTが成功を収めると，
ViTを用いた動作認識モデルが次々と提案された\cite{Selva_ArXiv2022_Video_Trans_Survey}．
ViTは画像をパッチに分割し，パッチをトークンとみなしてTransformerを適用するが，
ViTに基づく動作認識モデルは動画像をパッチに分割する．
この構造により，
時間情報の獲得の役割は自己アテンション機構が担うことになり，
また画像も動画像もまったく同様にTransformerへの入力として与えればよく，
モデルの設計が容易になった．


ここで問題となるのは計算コストである．
ViTの自己アテンション機構の計算量は$O(N^2)$である．
ここで$N$は入力パッチ数であり，
動画長が長くなるにつれてパッチ数を増やせば計算コストは増大してしまい，
逆にパッチ数を固定すると時間方向の解像度が落ちてしまう．
そのための対策も提案されているが\cite{Bertasius_ICML2021_TimeSformer,Bulat_NeurIPS2021_X-ViT}，
画像と動画像を同時に扱うためには適した方法ではない．
そこで本研究では，計算コストの低い効率的な
画像と動画像の同時学習モデルを提案する．
図\ref{fig:proposed model overview}に示す提案手法は，
フレーム毎に2次元画像認識モデル（ViT）を適用するという，
動作認識においてベースラインとしても用いられる単純な手法である\cite{Zhang_ACMMM2021_TokenShift}．
%
画像を認識する場合にはViTを適用し，
動画像を認識する場合にはlate fusion\cite{Karpathy_2014_CVPR}で各フレームに対するViTの出力を集約する．
%
この構造により，計算量を増やすことなくViTを用いた画像と動画像の同時学習が可能になる．
ただし時間情報をモデル化する必要があるため，
時間的特徴量シフトを用いる手法
\cite{Hashiguchi_2022_ACCVW_MSCA,Lin_2019ICCV_TSM,Zhang_ACMMM2021_TokenShift}
を適用する．
%
また画像と動画像というドメインの違いを吸収するために，
マルチドメイン学習・マルチデータセット学習の手法を適用する\cite{Li_2019_CVPR,Omi_IEICE-ED2022_MDL}．




本研究の貢献は以下の通りである．
\begin{itemize}
    \item 計算量の少ない，ViTを用いた画像と動画像の同時学習モデルを提案する．
    提案手法では単一の画像用ViTモデルを学習し，
    画像に対してはそのままViTを適用し，
    動画像に対してはフレーム毎にViTを適用し集約する．
    \item 画像と動画像の同時学習のために，時間的特徴量シフトを適用する．
    動作認識のために提案されたシフト手法を，
    画像と動画像の同時学習のために用いる研究は本研究が初めてである．
    \item 画像と動画像のドメインの違いを吸収するために，
    マルチドメイン学習手法を適用する方法を提案する．
    \item 複数の画像と動作認識のデータセットを用いて，
    画像と動画像の複数ドメインに対する性能を評価する．
\end{itemize}






\begin{figure}
\centering

\begin{minipage}[t]{0.6\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/method/method_image.pdf}
\subcaption{}
\end{minipage}

\vspace{2em}

\begin{minipage}[t]{0.8\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/method/method_video.pdf}
\subcaption{}
\end{minipage}

\caption{Schematic diagram of the proposed model based on ViT.
(a) When one image is entered．
(b) When a video clip consisting of $T$ frames is input.
}
\label{fig:proposed model overview}
\end{figure}


\section{関連研究}


\subsection{Image and Motion Recognition}

ImageNet \cite{Deng_CVPR2009_ImageNet}の登場以来，
画像認識分野において畳み込みニューラルネットワーク（CNN）を用いた手法が多数提案されており
\cite{He_2016_CVPR,Alex_NeurIPS2012_AlexNet,Simonyan_arXiv2014_VGG,Szegedy_arXiv2014_GoogLeNet}，
近年ではTransformer \cite{Vaswani_arXiv2017_transformer}を元にしたVision Transformer (ViT) \cite{Dosovitskiy_2021_ViT}
に基づいたモデルが多く提案されている\cite{Liu_2021_ICCV,Zhang_ACMMM2021_TokenShift}．
また，画像認識モデルの発展に伴い，動作認識の研究も盛んに行われており，
3次元CNNを用いた手法
\cite{Joao_CVPR2017_I3D,Feichtenhofer_CVPR2020_x3d,Feichtenhofer_ICCV2019_SlowFast,Hara_CVPR2018_3DResNet,Du_ICCV2015_C3D}
やViTに基づいた手法
\cite{Arnab_ICCV2021_ViVit,Bertasius_ICML2021_TimeSformer,Neimark_2021_ICCVW_VideoTransformerNetwork,Sharir_arxiv2021_STAM,Zhang_ACMMM2021_TokenShift}
が多数提案されている．
初期の研究には動画像の1フレームとオプティカルフローを用いる
Two-stream Network \cite{Karen_NeurIPS2014_TwoStream}
や，それを複数の動画区間に適用するTemporal Segment Network (TSN) \cite{Wang_ECCV2016_TSN}
なども提案されたが，
2D CNNを各フレームに適用して時間方向に集約するlate fusion \cite{Karpathy_2014_CVPR}
は処理が単純であり，ベースライン手法として比較に用いられることも多い．
しかし，late fusionだけでは時間方向のモデル化能力に限界があるため，
中間層の特徴を前後の時間でやり取りする
Temporal Shit Module (TSM) \cite{Lin_2019ICCV_TSM}
% やTokenShift \cite{Zhang_ACMMM2021_TokenShift}
% やMSCA \cite{Hashiguchi_arxiv2022_MSCA}
なども提案されている．

% Since the appearance of ImageNet \cite{Deng_CVPR2009_ImageNet}, many methods using convolutional neural networks (CNN) have been proposed in the field of image recognition. AlexNet,Simonyan_arXiv2014_VGG,Szegedy_arXiv2014_GoogLeNet}, and recently, Vision Transformer (ViT) based on Transformer \cite{Vaswani_arXiv2017_transformer} Recently, many models based on Transformer (ViT)\cite{Dosovitskiy_2021_ViT} based on Transformer \cite{Liu_2021_ICCV,Zhang_ACMMM2021_TokenShift} have been proposed. With the development of image recognition models, motion recognition has also been actively studied, and methods based on 3D CNNs \cite{Joao_CVPR2017_I3D,Feichtenhofer_CVPR2020_x3d,Feichtenhofer_ICCV2019_SlowFast, Hara_CVPR2018_3DResNet,Du_ICCV2015_C3D} and ViT-based methods \cite{Arnab_ICCV2021_ViVit,Bertasius_ICML2021_TimeSformer,Neimark_2021_ICCVW_ VideoTransformerNetwork,Sharir_arxiv2021_STAM,Zhang_ACMMM2021_TokenShift} have been proposed. Early work includes Two-stream Network \cite{Karen_NeurIPS2014_TwoStream}, which uses a single frame of video and optical flow, and Temporal Segment Network (TSN)\cite {Wang_ECCV2016_TSN} was also proposed, while late fusion \cite{Karpathy_2014_CVPR}, which applies a 2D CNN to each frame and aggregates it in the temporal direction, is a simple process and is often used as a baseline method for comparison. However, since late fusion alone is limited in its ability to model in the temporal direction, it is necessary to use a temporal shit module (TSM) that exchanges intermediate layer features back and forth in time, such as Temporal Shit Module (TSM)\cite{Lin_2019ICCV_TSM}% or TokenShift \cite{Zhang_2019ICCV_TSM}% or TokenShift{Zhang_2019ICCV_TSM}%. ACMMMM2021_TokenShift} % and MSCA \cite{Hashiguchi_arxiv2022_MSCA}} are also proposed.


\subsection{Simultaneous image and video learning}

このように画像認識モデルと動作認識モデルは別々に研究が行われていたが，
一つのモデルで画像と動画像の両方を識別する試みがいくつか行われている．
UniDual \cite{Wang_arXiv2019_UniDual}とOmnisorce \cite{Duan_arXiv2020_OmniSource}は，
静止画像を時間方向に複製して3次元ボリュームに変換することで，
SlowFast \cite{Feichtenhofer_ICCV2019_SlowFast}やR(2+1)D \cite{Tran_2018CVPR_R(2+1)D}などの
3D CNNモデルで統一的に扱う方法である．

CNNとは異なりViTはパッチ分割（tokenizer）を利用するため，
異なるモードのデータを統一的に扱いやすい．
これを利用したPolyVit \cite{Likhosherstov_arXiv2021_PolyViT}は画像・動画像・音声の，
Omnivore \cite{Girdhar_CVPR2022_Omnivore}は画像・動画像・3Dデータの
同時学習を行っており，
OmniMAE \cite{Girdhar_arXiv2022_OmniMAE}はパッチマスクによる画像・動画像の事前学習を
行っている．

これらの手法の問題点は，計算コストが増大することである．
静止画像を3次元ボリュームに変換する方法\cite{Duan_arXiv2020_OmniSource,Wang_arXiv2019_UniDual}
は不要な計算コストが発生してしまう．
またViTに基づく手法\cite{Girdhar_CVPR2022_Omnivore,Likhosherstov_arXiv2021_PolyViT,Girdhar_arXiv2022_OmniMAE}
の自己アテンション機構の計算量は$O(N^2)$であり，
動画が長くなれば入力パッチ数$N$が大きくなり，計算コストは増大してしまう．

一方で本研究は，
動画像に対してはフレーム毎にViTを適用してlate fusionで集約する．
また静止画像に対してはフレーム数1の動画像とみなすことで同じ処理を実現できる．
したがって動画像のフレーム数が多くなっても計算コストの増大はフレーム数に線形で抑えられる．


\section{手法}
本節では，より効率的な画像と動画の同時学習モデルを説明する．
ベースモデルとして，Vision Transformer (ViT) \cite{Dosovitskiy_2021_ViT}を使用する．
ただし，ViTはそのまま使用すると異なるモードの入力を同時に扱えない．
そこで，異なるモードの入力を同じにように扱うために，事前に，入力に対して変換を行う．
また，複数のデータセットで学習を行うため，ヘッドを複数用意する．

\subsection{画像用ViT}

ここではベースモデルに利用する元々の（画像用の）ViTを簡潔に説明する．

入力画像を$x \in \R^{3 \times H \times W}$とする．
ここで$H, W$は画像の高さと幅である．
入力画像はまずtokenizerによって
$P \times P$画素のパッチに分割され，
パッチ列のテンソル$\hat{x} = [x_0^1, \ldots, x_0^N] \in \R^{N \times d}$に変換される．
ここで$x_0^i \in \R^{d}$は$i$番目のパッチ，
$N = \frac{HW}{P^2}$はパッチ数，
$d = 3 P^2$はパッチ次元である．

入力パッチ$x_0^i$は$D$次元埋め込み行列$E \in \R^{d \times D}$による線形変換と
位置埋め込み$E_\mathrm{pos}$の加算により，以下のように変換される．
\begin{align}
    z_0 &= [c_0, x_0^1 E, x_0^2 E, \ldots, x_0^N E] + E_\mathrm{pos}
\end{align}
ここで$c_0 \in \R^{D}$はクラストークンである．
このパッチ埋め込み$z_0 \in \R^{(N+1) \times D}$が，
Transformerの最初のエンコーダブロック$M^\ell$へと入力される．

$z_\ell$を$\ell$番目のブロック$M^\ell$への入力，$z_\ell$を出力とすると，
ブロック内の処理は以下のように表現される．
\begin{align}
    z'_\ell &= \mathrm{MSA}(\mathrm{LN}(z_{\ell - 1})) + z_{\ell - 1}
    \\
    z_\ell &= \mathrm{MLP}(\mathrm{LN}(z'_\ell)) + z'_\ell,
\end{align}
ここでLNはレイヤー正規化，
MSAはマルチヘッド自己アテンション，
MLPは多層パーセプトロンである．
これを
\begin{align}
    z_{\ell} &= M^\ell (z_{\ell - 1})
\end{align}
と書くことにすると，$L$個のブロックからなるViTの出力$z_L$は
\begin{align}
    z_L = (M^L \circ M^{L-1} \circ \cdots M^1 \circ M^0) (x)
    \in \R^{(N+1) \times D}
\end{align}
と表せる．ただし
$\circ$は関数合成，
$M^0$はtokenizerとする．
これに対して線形層とsoftmaxからなるヘッド$M^h$を適用することでクラス予測
\begin{align}
    \hat{y} &= M^h(z_L)
\end{align}
を得る．

ただし通常は$z_L$のうちクラストークンに対応する部分だけが利用される．
$z_\ell$の$(n,d)$要素を$z_{\ell, n, d}$，
クラストークンに対応する部分$\tilde{z}_\ell \in \R^D$の要素を
$\tilde{z}_{\ell, d}$と表すとすると
\begin{align}
    \tilde{z}_{\ell, d} &= z_{\ell, 0, d}
\end{align}
に対して
\begin{align}
    \hat{y} &= M^h(\tilde{z}_L) \in [0, 1]^C
\end{align}
である．ここで$C$はカテゴリ数である．



\subsection{フレーム毎の動画用ViT}

フレーム毎に画像用のViTを適用する
\cite{Hashiguchi_2022_ACCVW_MSCA,Zhang_ACMMM2021_TokenShift}
ために，上述の定式化を修正する．

入力動画像クリップを$x \in \R^{T \times 3 \times H \times W}$とする．
ここで$T$は動画クリップ中のフレーム数である．
各フレームがtokenizerによって
$P \times P$画素の$N$個のパッチ
$\hat{x} = [x_0^1, \ldots, x_0^N] \in \R^{T \times N \times d}$
に変換される．
ここで$x_0^i \in \R^{T \times d}$はフレーム内の$i$番目のパッチである．

パッチ埋め込みは画像の場合と同様に以下のようになる．
\begin{align}
    z_0 &= [c_0, x_0^1 E, x_0^2 E, \ldots, x_0^N E] + E_\mathrm{pos}
\end{align}
ただしクラストークンの次元は$c_0 \in \R^{T \times D}$，
パッチ埋め込みの次元は$z_0 \in \R^{T \times (N+1) \times D}$となる．

これを$L$個のブロック$M^{\ell}$からなるViTへ入力して得られる出力$z_L$は
\begin{align}
    z_L = (M^L \circ M^{L-1} \cdots M^1 \circ M^0) (x)
    \in \R^{T \times (N+1) \times D}
\end{align}
である．

この$T$フレーム分の出力を集約する方法には色々考えられるが\cite{Sharir_arxiv2021_STAM}，
本研究では最も簡単な時間的平均プーリングを用いる\cite{Hashiguchi_2022_ACCVW_MSCA,Zhang_ACMMM2021_TokenShift}．
$z_\ell$の$(t,n,d)$要素を$z_{\ell,t, n, d}$，
クラストークンに対応する部分$\tilde{z}_\ell \in \R^{T \times D}$の要素を
$\tilde{z}_{\ell, t, d}$と表すとすると，クラストークン部分
\begin{align}
    \tilde{z}_{\ell, t, d} &= z_{\ell, t, 0, d}
\end{align}
に対する平均プーリングは
\begin{align}
    \bar{z}_{\ell, d} &= \frac{1}{T} \sum_t^T \tilde{z}_{\ell, t, d}
\end{align}
であり，これに対してヘッドを適用して得られる予測は
\begin{align}
    \hat{y} &= M^h(\bar{z}_L) \in [0, 1]^C
\end{align}
である．







\subsection{提案モデル}

前述の画像用と動画用のViTはバッチ単位の処理によって統一的に扱うことができる．
一般的にモデルへの入力は，$B$毎の画像を束ねたバッチサイズ$B$のバッチ
$x \in \R^{B \times 3 \times H \times W}$であり，
それに対する出力$\hat{y} \in [0, 1]^{B \times C}$もバッチ単位である．
つまり上記のViTのブロック$M_\ell$の入出力も
$z_\ell \in \R^{B \times (N+1) \times D}$
となる．
したがって，
動画像のフレームが入力なのか，
それとも画像のバッチが入力なのかを，
ブロック側では区別する必要がない．

そこで以下のように，画像と動画像とで入力と出力の扱いを変更することで，
同じViTブロックを画像と動画に適用する．




\subsubsection*{画像の入力}

画像のバッチ
$x \in \mathbb{R}^{B \times 3 \times H \times W}$
を入力とする．
第$L$ブロックの出力は
$z_L \in \R^{B \times (N+1) \times D}$
であり，そのクラストークン部分
$\tilde{z}_L \in \R^{B \times D}$
をヘッドで識別した出力は
$\hat{y} \in [0, 1]^{B \times C}$
である．

これは画像用ViTでバッチを扱う場合の同様の処理である．



\subsubsection*{動画の入力}

動画像クリップのバッチ
$x \in \mathbb{R}^{B \times T \times 3 \times H \times W}$
を入力とする．
この5次元テンソルをViTへ入力するために，フレーム次元をバッチ次元へと展開して
4次元テンソル$x' \in \mathbb{R}^{BT \times 3 \times H \times W}$と変形する．



第$L$ブロックの出力は$z_L \in \mathbb{R}^{BT \times (N+1) \times D}$であり，
これをまず
$z'_L \in \mathbb{R}^{B \times T \times (N+1) \times D}$へと変換する．
そしてクラストークン部分
$\tilde{z}'_L \in \mathbb{R}^{B \times T \times D}$を取り出して，
平均プーリングを適用して
$\bar{z}'_L \in \mathbb{R}^{B \times D}$を得る．
これをヘッドで識別した出力は
$\hat{y} \in [0, 1]^{B \times C}$
である．



\subsection{実装における課題}

上記のように画像と動画像を入力にとるモデルを実装する際に，
考慮するべき事項が多数存在する．

\subsubsection{事前学習済みモデルの重み}

データセットサイズが小さい場合に，大規模データセットで事前学習したモデルの
重みを初期値として利用することは一般的に行われている．
画像認識においてはImageNet-1kや21kで事前学習した重みを用いることが標準的であり，
動作認識ではKinetics-400で事前学習した重みを用いることが多い．
しかし本研究では同じモデルで画像と動画像を識別するため，
事前重みは画像と動画像の両方に有効である必要がある．
そのためには重みの事前学習に画像と動画像のどちらのデータセットを用いれば
有効であるのかを調査する必要がある．



実験ではViTを
ImageNet-21kで事前学習した重み
\footnote{\url{https://github.com/lukemelas/PyTorch-Pretrained-ViT}}と，
フレーム毎にViTを適用するモデルを
Kinetics-400で事前学習した重み
\footnote{\url{https://github.com/VideoNetworks/TokShift-Transformer}}
を用いた場合の性能を比較する．


\subsubsection{ハイパーパラメータの選定}

データセット毎に最適なハイパーパラメータが異なるため，
各データセットで別々の最適化手法，異なる学習率や重み減衰の値を
使用することも多い\cite{Likhosherstov_arXiv2021_PolyViT}．
しかし画像と動画像を同一のモデルで扱う場合，
別々のモダリティであるにも関わらず
同じハイパーパラメータが適切であるとは限らない．
さらに複数の画像や動画像データセットを扱う場合には，
すべてのデータセットに対して適切なハイパーパラメータを探索することは
現実的ではなく，
またそれぞれのデータセットに最適なハイパーパラメータを求めたとしても
複数データセットでの学習時にも有効であるとは限らない．


そこで本研究では以下のハイパーパラメータ設定を実験において比較する．


\begin{itemize}
\item all：Unify settings for all datasets. Even if there are multiple image datasets or multiple video datasets, use the same settings for all of them.

\item domain：The settings are standardized for images and videos, respectively. Multiple image datasets use common settings among them, and multiple video datasets use common settings among them. However, images and videos do not necessarily share the same settings.

\item each：Use separate settings for each dataset. Use separate settings for each dataset.
Separate experiments are conducted to determine the value, and the appropriate value is used when each dataset is trained separately.
\end{itemize}




\begin{figure}
\centering

\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/all.pdf}
\subcaption{}
\end{minipage}
\hfil
\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/domain.pdf}
\subcaption{}
\end{minipage}
\hfil
\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/each.pdf}
\subcaption{}
\end{minipage}

\caption{Various settings for optimizer methods．
(a) all：To unify all data sets．
(b) domain：When unified with image and video data sets．
(c) each：To set for each data set．
}
\label{fig:hyperparameter selection}
\end{figure}




\subsubsection{時間情報のモデル化}

提案手法では動画像をフレーム毎にViTで特徴量抽出を行い，
それを時間方向への平均プーリングを適用することで，動画単位の予測を行う．
しかしこのフレーム毎のViTのままでは動画像の時間情報のモデル化能力が弱い．
そこで，この構造を維持したまま時間情報を扱うことのできる手法を導入する．
具体的には，TSM \cite{Lin_2019ICCV_TSM}をViTに導入した
TokenShift \cite{Zhang_ACMMM2021_TokenShift}と
MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}を用いる．



\begin{figure}[t]

    \centering
    
    
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/ViT.pdf}\\
    \subcaption{}
    \label{fig:ViT_block}
    \end{minipage}
    \hfil
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/tokenshift.pdf}
    \subcaption{}
    \label{fig:tokenshift_block}
    \end{minipage}
    \hfil
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/MSCA.pdf}
    \subcaption{}
    \label{fig:MCSA_block}
    \end{minipage}

    
    \caption{
    Encoder block for each model．
    (a) ViT \cite{Dosovitskiy_2021_ViT}，
    (b) TokenShift \cite{Zhang_ACMMM2021_TokenShift}，
    (c) MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}．
    }
    \label{Fig:overview}

\end{figure}

これらの手法では，$\ell$番目のブロック$M^\ell$において，
$z_{\ell, t, n, d}$の時間次元$t$に対して，
前後の時刻の特徴である
$z_{\ell, t+1, n, d}$と$z_{\ell, t-1, n, d}$を
用いて，特徴量シフト\cite{Zhang_ACMMM2021_TokenShift}
またはアテンションのシフト\cite{Hashiguchi_2022_ACCVW_MSCA}を行う．
この方法では1つのブロックが1時刻分だけ情報を
時間方向へ伝播させる．
そのため，
入力動画像クリップ長が$T$フレームであれば，
ブロック数を$L \ge T$とすることで，
全時刻分の時間情報の相互作用することが
できることが示されている\cite{Hashiguchi_2022_ACCVW_MSCA}．



\subsubsection{損失関数の重み付け}

データセットが異なると一般にカテゴリ数も異なる．
そのため，ヘッドはデータセット毎に用意する
マルチヘッドの構造を取ることが一般的である\cite{Omi_IEICE-ED2022_MDL}．
$i$番目のデータセットを$\mathcal{D}_i$，
カテゴリ数を$C_i$，
ヘッドを$M^h_i$，
このヘッドに付随する損失関数を$\mathcal{L}_i()$とする．

本手法では，モデルへ入力するバッチはある一つのデータセットからサンプリングする．
つまりあるバッチのデータとその教師ラベルのペアを
$(x, y)$とすると，損失関数は次のようになる\cite{Omi_IEICE-ED2022_MDL}．
\begin{align}
    \mathcal{L}
    &=
    E_{\mathcal{D}_i \sim \mathcal{D}}
    E_{ (x, y) \sim \mathcal{D}_i}
    \left[ \mathcal{L}_i( \hat{y}, y ) \right]
\end{align}
ここで$\mathcal{D} = \{ \mathcal{D}_1, \ldots, \mathcal{D}_{D_N} \}$
は$D_N$個のデータセット集合である．

データセットのサンプリングはいろいろな方法が考えられるが，
データセットサイズに比例してサンプルを取得する方法が性能が良い
ということが報告されている\cite{Likhosherstov_arXiv2021_PolyViT}．
本研究ではサンプリングの代わりに，以下のように
データセット毎の損失関数の重み付け和とバッチ単位の経験損失で近似することを考える．
\begin{align}
    \mathcal{L}
    &=
    \sum_{i=1}^{D_N}
    w_i
    \mathcal{L}_i \\
    \mathcal{L}_i
    &=
    \frac{1}{S_i}
    \sum_{b=1}^{S_i}
    \mathcal{L}_i( \hat{y}_b, y_b )   
\end{align}
ここで$S_i$はデータセット$i$からサンプルできるバッチ数
（データ数はこれにバッチサイズを乗じたものになる），
$\hat{y}_b, y_b$はバッチ$b$の予測と真値のラベルである．
実際のバッチ単位の更新では重みをバッチ単位の損失に組み込んだ
\begin{align}
    w_i \mathcal{L}_i( \hat{y}_b, y_b )   
\end{align}
を用いて勾配計算を行う．

ここで重み$w_i$として，マルチタスク学習
\cite{Crawshaw_arXiv2020_Multi-Task_survey,Vandenhende_TPAMI2022_Multi-Task_survey}
で提案されている
2つの手法を用いる．
マルチタスク学習においては，タスク毎に学習が進む速度が異なるため，
その学習速度を重みによって制御する必要がある．
本研究においては，動画像は複数フレームを持つため，画像よりも学習の収束が遅いと
考えられる．そこで，データセットサイズに依存する単純な固定重みではなく，
学習進度に依存する重みを導入することにより，データセット毎の学習速度の差を緩和させる．


\begin{description}

\item[Dynamic Task Prioritization (DTP)
    \cite{Guo_2018ECCV_Dynamic_Task_Prioritization}]
データセットの学習度合いに応じて重み$w_i$を次式で定義する．
\begin{align}
    w_i(t) = - (1 - \kappa_i(t))^{\gamma_i} \log{\kappa_i(t)}
\end{align}
ここで$\kappa_i(t)$はデータセット$i$に対する$t$回目の反復における性能指標，
$\gamma_i$は損失に対する重み（focusing parameter）\cite{Lin_2017_ICCV_focal_loss}，
$t$は反復回数（バッチ数）である．


\item[Dynamic Weight Averaging (DWA)
      \cite{Liu_2019CVPR_DWA_Dynamic_Weight_Averaging}]
直近の損失関数値の減少度合いに応じて重み$w_i$を次式で定義する．
\begin{align}
    w_{i}(t) &= \frac{N\exp(r_i(t-1)/T)}{\sum_{n=1}^{D_N}{\exp(r_n(t-1)/T)}} \\
    r_i(t-1) &= \frac{\mathcal{L}_i(t-1)}{\mathcal{L}_i(t-2)}
\end{align}
ここで$D_N$はデータセット数，
$T$は温度パラメータ，
$\mathcal{L}_i(t)$はデータセット$i$に対する$t$回目の反復における損失値，
$t$は反復回数（バッチ数）である．
\end{description}

なおマルチタスク学習
\cite{Crawshaw_arXiv2020_Multi-Task_survey,Vandenhende_TPAMI2022_Multi-Task_survey}
では，1つのサンプルに対して複数の損失関数の計算が発生するが，
マルチドメイン学習\cite{Omi_IEICE-ED2022_MDL}や
マルチデータセット学習\cite{Liang_NeurIPS2022_Multi-Dataset}では，
あるサンプルに対して計算する損失関数は1つである．




%%%%%%%%%%%%%%%%%% 事前重みの選定の実験 %%%%%%%%%%%%%%%%%%%

\begin{figure*}

    \centering

    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/TinyI.pdf}
        \subcaption{Tiny-ImageNet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/CIFAR100.pdf}
        \subcaption{CIFAR100}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/UCF101.pdf}
        \subcaption{UCF101}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/K200.pdf}
        \subcaption{mini-Kinetics}
    \end{minipage}

    \caption{各データセット個別の学習における，
    ImageNet-21k（I21k）とKinetics400（K400）での事前学習済み重みを用いた場合の性能の比較
    }
    \label{fig:pretrain}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{実験}

提案手法を評価するために，複数のデータセットを用いた実験を行い，
各種設定の性能の比較を行った．


\subsection{実験設定}

\subsubsection*{データセット}

実験では，
以下の2種類の画像データセットと2種類の動画データセットを用いる．
つまりドメインは画像と動画像の2つ，合計データセット数は$D_N=4$である．

\begin{itemize}

\item Tiny-ImageNet \cite{Tiny_ImageNet_kaggle2018}：
10万枚の学習用画像，1万枚の検証用画像から構成される画像データセット．
各学習画像は，ImageNet \cite{Deng_CVPR2009_ImageNet}の200クラス（各クラス500枚）から抽出された$64 \times 64$画素の画像である．

\item CIFAR-100 \cite{Krizhevsky_TR2009_CIFAR10-100}：
5万枚の学習用画像，1万枚の検証用画像から構成される画像データセット．
カテゴリ数は100，画像サイズは$32 \times 32$である．

\item Mini-Kinetics (Kinetics-200) \cite{Xie_2018ECCV_S3D_Kinetics200}：
78246本の学習用動画像と5000本の検証用動画像から構成される動作認識データセット．
各動画像はKinetics-400の200クラス（各クラス400本程度）から抽出されたものである.

\item UCF101 \cite{Soomro_arXiv2012_UCF101}：
9537本の学習用動画像と3783本の検証用動画像からなる101クラスの動作認識データセット.

\end{itemize}

いずれのデータセットについても，
性能評価には検証セットのtop-1（val top-1）を用いる．





\subsubsection*{モデル}

実験では，
提案手法，
TokenShift \cite{Zhang_ACMMM2021_TokenShift}, 
MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}の
ベースモデルにVision Transformer \cite{Dosovitskiy_2021_ViT}を使用する．
ヘッドはデータセット毎に存在するため，各モデルは4つのヘッドを持つ．

\subsubsection*{学習サンプル}

画像データセットについては，1枚の画像に対して，
元の画像の$[0.08, 1.0]$倍の範囲のサイズをランダムにクロップし，
アスペクト比を$[\frac{3}{4}, \frac{4}{3}]$の範囲でランダムに決定し，
$224 \times 224$画素にリサイズを行う．
その後，$1/2$の確率で水平方向に反転をさせる．


動画データセットについては，1つの動画から指定した秒数（クリップ時間）に相当する連続するフレームを抽出し，そこから時間方向に均一に16フレームをサンプリングして1クリップを作成する．
サンプリングレートはデータセット（と動画）によって異なるが，
実験ではクリップ時間を約2.67 秒に固定した．
取り出したフレームの短辺を$[224, 320]$画素の範囲でランダムに決定し，
アスペクト比を保ったままリサイズする．
その後ランダムな場所の$224 \times 224$画素をクロップし，
$1/2$の確率で水平方向に反転させる．




\subsubsection*{バッチサンプリング}

複数データセットを同時学習する際には，
どの順番でデータセットからバッチをサンプルして学習するか，
データセット毎にどの割合でバッチをサンプルするかなど考慮する必要がある
\cite{Likhosherstov_arXiv2021_PolyViT}．
本手法では\cite{Omi_IEICE-ED2022_MDL}と同様の手順でバッチをサンプリングしパラメータを更新する．


\begin{itemize}
\item 
データセットサンプリング順は固定とし，
Tiny-ImageNet，CIFAR100，UCF101，mini-Kineticsの順で行う．

\item
それぞれのデータセットにおいて，バッチサイズは6に固定し，
1バッチずつサンプルする．
したがって画像データセットのミニバッチは6枚の画像からなり，
動画像データセットのミニバッチは，6本の動画像のそれぞれが16フレームからなるため，
96フレームからなる．

\end{itemize}


各データセットからミニバッチをサンプリングし，勾配を計算し，パラメータ更新を行う．これを1反復とする．





\subsection{事前学習済みモデルの重みの選定}

まず
各データセットでの個別の学習において，
ベースモデルであるViTの重みを，
ImageNet-21kで事前学習した重みを利用した場合と，
Kinetics400で事前学習した重みを利用した場合との
性能を比較する．
学習反復回数は50000に固定した．
最適化手法はいずれもSGD，学習率は画像データセットでは1e-4，
動画データセットでは1e-3とした．
その他のパラメータのデフォルト値を表\ref{Tab:default}に示す．





結果を図\ref{fig:pretrain}に示す．
画像データセットであるTiny-ImageNetやCIFAR100に対しては，
最終的にはKinetics400とImageNet-21kのどちらの重みを
利用しても性能には差がなくなるものの，
学習初期段階ではKinetics400の重みのほうが性能が高い．
一方の動画データセットであるUCF101やmini-Kineticsに対しては，Kinetics400の重みのほうが
一貫して性能が高いことがわかる．
以上より，以降の実験においてはKinetics400で事前学習した重みを採用する．


%%%%%%%%%%% 最適化手法のデフォルト値 %%%%%%%%%%%
\begin{table}[t]
  \centering
  \caption{各最適化手法のデフォルト値}
  \label{Tab:default}

\scalebox{0.8}{
  \begin{tabular}{c|cccc}
     & 重み減衰 & モーメンタム & $ \beta_1 $ & $ \beta_2 $ \\
     \hline
     SGD & 5e-5 & 0.9 & -- & -- \\
     Adam & 5e-5 & -- & 0.9 & 0.999 \\
     AdamW & 5e-5 & -- & 0.9 & 0.999 
  \end{tabular}
}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%% optimizer選定の事前実験の性能図 %%%%%%%%%%%%%%%%%
\begin{figure*}

    \centering
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/TinyI.pdf}
        \subcaption{Tiny-ImageNet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/CIFAR100.pdf}
        \subcaption{CIFAR100}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/UCF101.pdf}
        \subcaption{UCF101}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/K200.pdf}
        \subcaption{mini-Kinetics}
    \end{minipage}
    
    \caption{各データセット個別の学習における，
    9つの最適化手法，学習率の性能の比較
    }
    \label{fig:dataset_opt_acc}
\end{figure*}



\begin{table*}[t]

  \centering
  \caption{各データセットでの個別の学習において最適化と学習率を
  変更した場合の性能の比較．}
  \label{Tab:dataset_opt_acc}

 
\begin{tabular}{cc|cccccccc}
 \multicolumn{2}{c}{} &  \multicolumn{2}{c}{Tiny-ImageNet} & \multicolumn{2}{c}{CIFAR100} &  \multicolumn{2}{c}{UCF101} &  \multicolumn{2}{c}{mini-Kinetics} \\
optimizer & lr & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ 
\hline
Adam & 1e-3 & \phantom{0}6.95 & 21.39 & 15.19 & 41.27 & 16.8 & 43.41 & \phantom{0}2.66 & 88.54 \\
     & 1e-4 & 68.11 & 88.05 & 80.94 & 96.80 & 76.19 & 93.07 & 24.12 & 53.64\\
     & 1e-5 & \textbf{81.90} & 94.30 & 88.89 & 98.81 & 87.43 & 98.04 & \textbf{68.26} & 88.68 \\
\hline
AdamW & 1e-3 & \phantom{0}0.50 & \phantom{0}2.50 & \phantom{0}9.35 & 29.70 & 0.85 & \phantom{0}4.81 & \phantom{0}0.50 & \phantom{0}2.50 \\
      & 1e-4 & 70.33 & 89.54 & 81.66 & 97.10 & 79.42 & 93.60 & 58.58 & 82.98 \\
      & 1e-5 & 81.27 & 94.36 & \textbf{89.19} & 98.77 & 88.15 & 97.86 & 68.20 & 88.40 \\
\hline
SGD & 1e-3 & 81.60 & 94.85 & 87.90 & 98.56 & \textbf{90.50} & 98.81 & 66.82 & 87.96 \\
    & 1e-4 & 79.78 & 93.53 & 88.04 & 98.68 & 87.59 & 98.62 & 66.90 & 88.06\\
    & 1e-5 & 14.78 & 33.80 & 57.31 & 83.68 & 62.91 & 88.54 & 16.56 & 36.06 \\

\end{tabular}


\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\subsection{ハイパーパラメータの設定方法}

次に複数のデータセットの同時学習において，
最適化手法とハイパーパラメータを
全データセットで統一した場合（all），
画像，動画で統一した場合（domain）
各データセットで個別に設定した場合（each），
の性能を比較する．
本実験では，
最適化手法を
SGD，
Adam \cite{Kingma_ICLR2015_Adam}，
AdamW \cite{Loshchilov_ICLR2019_AdamW}
の3種類，
ハイパーパラメータを学習率のみに限定し1e-3，1e-4，1e-5の3種類，
合計9通りの設定での性能を比較する．


ただしすべての設定の組み合わせを比較することは
現実的ではないため，
まず各データセットでの個別の学習において有効な設定を
事前実験によって求め，
それを基にall，domain，eachの設定を決定する．



\subsubsection*{事前実験}

各データセットでの個別の学習を，
前述の9通りの設定で行った結果を
図\ref{fig:dataset_opt_acc}と
表\ref{Tab:dataset_opt_acc}に示す．
学習反復回数は50000，その他の設定は前述の通りとした．


\begin{itemize}

\item 
(Adam, 1e-3), (AdamW, 1e-3), (SGD, 1e-5)の組み合わせは
どのデータセットに対しても良い性能が得られておらず，
一方で(Adam, 1e-5), (AdamW, 1e-5), (SGD, 1e-3), (SGD, 1e-4)は
どのデータセットでも性能が良いことが分かる．
データセット毎に最も性能が良かった組み合わせは，
Tiny-ImageNetは(Adam, 1e-5)，
CIFAR100は(AdamW, 1e-5)，
UCF101は(SGD, 1e-3)，
mini-Kineticsは(Adam, 1e-5)
であり，
これらをeachの設定として採用する．

\item
画像と動画それぞれで比較すると，
画像データセットであるTiny-ImageNetとCIFAR100に対しては
(Adam, 1e-5)の性能が比較的高く，
動画データセットであるUCF101とmini-Kineticsに対しては
(AdamW, 1e-5)の性能が比較的高い．
そこでdomainの設定にはこれらを採用する．

\item
allの設定には，
全データセットに平均的に有効な(AdamW, 1e-5)を採用する．
\end{itemize}

以上より，選定した3つの場合の設定を表\ref{Tab:optimizer}に示す．

\begin{table*}[t]
  \centering
  \caption{all，domain，eachのそれぞれの場合の学習に用いた最適化手法と学習率．}
  \label{Tab:optimizer}

  \begin{tabular}{c|cccccccc}
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Tiny-ImageNet} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{UCF101} & \multicolumn{2}{c}{mini-Kinetics} \\
    setting & optimizer & lr & optimizer & lr & optimizer & lr & optimizer & lr \\
    \hline
    all     & AdamW & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 \\
    domain  & Adam & 1e-5 & Adam & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 \\
    each    & Adam & 1e-5 & AdamW & 1e-5 & SGD & 1e-3 & Adam & 1e-5 \\
    
  \end{tabular}
\end{table*}





\subsubsection*{学習}
上述の事前実験で選定した設定を用いて，all，domain，eachの場合の比較を行う．
学習反復回数は100000，バッチサイズは4とする．
ViTベースモデルの重みはKinetics400で事前学習したものを用いる．


結果を図\ref{fig:optimizer}に示す．
allの場合（図\ref{fig:optimizer all}）は，
どのデータセットも最終的に学習が成功している．
それに対して
domainの場合（図\ref{fig:optimizer domain}）と
eachの場合（図\ref{fig:optimizer each}）は，
学習に失敗しているデータセットがある．
このことは，複数のデータセットを同時に学習する場合には，
データセット個別で学習した場合とは，
適したハイパーパラメータの設定が異なることを示唆している．
他の値を用いた設定ではdomainとeachの場合も学習が成功する可能性はあるが，
本研究では以降の実験ではallの設定を用いる．


%%%%%%%%%%%%%%%% 最適化手法の選定の性能図，表 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/all_graph.pdf}
        \subcaption{all}
        \label{fig:optimizer all}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/domain_graph.pdf}
        \subcaption{domain}
        \label{fig:optimizer domain}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/each_graph.pdf}
        \subcaption{each}
        \label{fig:optimizer each}
    \end{minipage}

    \caption{
    ハイパーパラメータの設定の違いによる性能の比較．
    }
    \label{fig:optimizer}
\end{figure*}



\begin{table*}[t]

  \centering
  \caption{ハイパーパラメータの設定の違いによる性能の比較．averageは各データセットの性能の単純平均．}
  \label{tab:optimizer}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  setting & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
  
all    & 82.80 & 95.02 & 89.48 & 98.74 & 90.79 & 98.76 & 67.94 & 88.12 & 82.75 & 95.16 \\
domain & 80.78 & 94.05 & \phantom{0}5.86 & 26.68 & \phantom{0}7.75 & 20.29 & \phantom{0}1.44 & \phantom{0}6.80 & 23.96 & 36.96\\
each   & 76.60 & 92.81 & 84.85 & 97.84 & 83.84 & 96.27 & \phantom{0}5.10 & 15.34 & 62.60 & 75.57\\
\end{tabular}


\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{時間情報のモデル化の比較}

次に，単純なフレーム毎のViTと，
時間情報をモデル化する
TokenShift \cite{Zhang_ACMMM2021_TokenShift}と
MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}を
を用いた場合の性能を比較する．
すべての学習設定は，前項で選定したallの場合と同一である．

結果を図\ref{fig:temporal models}に示す．
どのモデルも学習は安定しており，性能に大きな差はないことが分かる．
表\ref{tab:temporal models}は，
図\ref{fig:temporal models}の学習終了時の性能である．
TokenShiftの性能が他の2つのモデルよりも平均の性能が高く，
またデータセット毎の性能でもTiny-ImageNet以外は性能が高い．
特に動画データセットであるUCF101では約1\%の差がある．
以上より，次の実験においてはベースモデルにTokenShiftを用いる．



\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/all_graph.pdf}
        \subcaption{ViT}
        \label{fig:temporal model ViT}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/tokenshift_result.pdf}
        \subcaption{TokenShift}
        \label{fig:temporal model TokenShift}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/MSCA_result.pdf}
        \subcaption{MSCA}
        \label{fig:temporal model MSCA}
    \end{minipage}

    \caption{
    時間情報のモデル化の違いによる性能の比較．学習設定はall．
    \subref{fig:temporal model ViT}は図\ref{fig:optimizer all}と同一である．
    }
    \label{fig:temporal models}
\end{figure*}


\begin{table*}[t]

  \centering
  \caption{時間情報のモデル化の違いによる性能の比較．averageは各データセットの性能の単純平均．}
  \label{tab:temporal models}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
ViT        & 83.55 & 95.06 & 88.89 & 98.80 & 90.42 & 98.39 & 67.78 & 87.58 & 82.66 & 94.96 \\
TokenShift & 83.29 & 95.14 & 89.37 & 98.72 & 91.24 & 98.65 & 67.82 & 88.74 & 82.93 & 95.31 \\
MSCA       & 82.51 & 94.96 & 89.12 & 98.68 & 89.97 & 98.92 & 66.58 & 86.98 & 82.05 & 94.89 \\
\end{tabular}


\end{table*}











\subsection{損失の重み付け方法の選定}

次に，複数データセットの損失に動的な重み付けを行わない場合（$w_i=1$），
DTP \cite{Guo_2018ECCV_Dynamic_Task_Prioritization}を用いた場合，
DWA \cite{Liu_2019CVPR_DWA_Dynamic_Weight_Averaging}を用いた場合を比較する．

学習反復回数は100000，バッチサイズは4とする．
モデルはTokenShift，事前重みはKinetics400 pretrained，
ハイパーパラメータはallと同様の設定とする．
DTPの性能指標$\kappa_i(t)$には各データセットの学習セットに対するtop-1性能の
過去500反復分（全データセット2000反復分のうち対応するデータセットの更新分のみ）の平均を用い，
focusing parameterは全データセット共通で$\gamma_i = 1$とした．
DWAの温度パラメータは$T = 1$とし，
損失$L(t)$には各データセットの学習セットに対する損失の過去500反復分（同上）の平均を用いた．


結果を図\ref{Fig:loss_weighting}に示す．
図\ref{Fig:loss_weighting}は，各場合におけるaccuracyの推移を表しており，
図\ref{fig:static loss weight}は前章のTokenShift（図\ref{fig:temporal model TokenShift}）と同一である．

DWA，DTPを用いた場合（図\ref{fig:DWA loss weight}，図\ref{fig:DTP loss weight}）と
しない場合（図\ref{fig:static loss weight}）とでは，
学習推移に大きな差はなく，学習は安定している．
表\ref{tab:loss_weighting}に図\ref{Fig:loss_weighting}の学習終了時の結果を示す．
DTPを用いた場合は平均の性能が重み付けなしの場合よりも下がっており，
DWAを用いた場合が最も性能が高かった．


%%%%%%%%%%%%%%%%%%%%% lossの重みづけの性能図，表 %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/tokenshift_result.pdf}
        \subcaption{static weight}
        \label{fig:static loss weight}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/loss/dwa.pdf}
        \subcaption{DWA}
        \label{fig:DWA loss weight}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/loss/task_prio.pdf}
        \subcaption{DTP}
        \label{fig:DTP loss weight}
    \end{minipage}

    \caption{
    損失の重み付け方法の違いによる性能の比較．
    モデルはTokenShift，学習設定はall．
    \subref{fig:DWA loss weight}は
    図\ref{fig:temporal model TokenShift}と同一である．    
    }
    \label{Fig:loss_weighting}
\end{figure*}




\begin{table*}[t]

  \centering
  \caption{損失の重み付け方法の違いによる性能の比較．averageは各データセットの性能の単純平均．}
  \label{tab:loss_weighting}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
static  & 83.29 & 95.14 & 89.37 & 98.72 & 91.24 & 98.65 & 67.82 & 88.74 & 82.93 & 95.31 \\
DWA     & 83.76 & 95.41 & 89.40 & 98.83 & 90.82 & 98.73 & 68.44 & 88.12 & 83.11 & 95.27 \\
DTP     & 80.80 & 94.49 & 87.80 & 98.47 & 89.05 & 98.54 & 62.28 & 85.44 & 79.98 & 94.24 \\
\end{tabular}


\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{おわりに}

本稿では，画像と動画像を同じモデルで扱うことのできるモデルを提案し，
その学習手法を検討した．
今後の課題として，動画像をフレーム分割したことで失われた時間情報を扱う別のモデルの採用，
動画像識別における平均プーリングによる単純なlate fusionの変更等がある．







==> main_text_eng.tex <==

\section{introduction}

With the recent development of deep learning, various tasks have been studied.
Among them, image recognition and action recognition have been studied extensively. 
Image recognition is a long-standing task, and many deep learning models have been proposed. 
Many deep learning models have been proposed\cite{Dosovitskiy_2021_ViT,He_2016_CVPR, Alex_NeurIPS2012_AlexNet,Simonyan_arXiv2014_VGG,Szegedy_arXiv2014_GoogLeNet}, and many datasets for image recognition have been made publicly available\cite{Deng_IEEE2009_ImageNet, Lecun_IEEE1998_MNIST}.
action recognition research also has a long history\cite{Kensho_IMP2020_video_recog_3D_conv, Yu_2022_human_action_recog,Zhu_arXiv2020_comprehensive}, with large datasets\cite{Kuehne_ICCV2011_HMDB51, Li_arXiv2020_AVA-Kinetics,Soomro_arXiv2012_UCF101} and various models\cite{Arnab_ICCV2021_ViVit, Joao_CVPR2017_I3D,Feichtenhofer_CVPR2020_x3d,Feichtenhofer_ICCV2019_SlowFast,Hara_CVPR2018_3DResNet,Karen_NeurIPS2014_TwoStream,Du_ICCV2015_C3D,Zhang_ACMMM2021_TokenShift} proposed. 
The type of data handled, such as images and videos, is called a mode, and methods that handle multiple modes are called multimodal or cross-modal. 
Major modes include natural language and speech, as well as image and video. 
Compared to the pre-deep learning era, it is relatively easy to study multimodal methods that simultaneously learn language or speech and image/video, and there are many multimodal methods that deal with image, video and text\cite{Aafaq_arXiv2018_Video_captioning_survey, Stefanini_arXiv2021_Video_Caption}, image, video and speech\cite{Zhang_CVPR2022, Zhu_arXiv2020_Audio_survey}, and video and speech\cite{Jaegle_ICML2021_Perceiver}.


Since images and video are often regarded as similar modes compared to language and audio, there have been few multimodal studies that deal with images and video at the same time. On the other hand, domain adaptation has been studied extensively for both images and videos\cite{redko_arXiv2020,wang_Elsevier2018,wilson_arXiv2020}. 


Domains are trends or features that are specific to a dataset, and models usually need to be re-trained for different domains or datasets. 
Domain adaptation is a general term for methods that allow the same model to be used across two different domains. 
Multi-domain learning\cite{Li_2019_CVPR,Omi_IEICE-ED2022_MDL,Rebuffi_2018_CVPR} and multi-dataset learning\cite{Liang_NeurIPS2022_Multi-Dataset,Zhou_2022_CVPR} are methods that train a single model on data from multiple different domains.
 
With the rapid adoption of Vision Transformer (ViT)\cite{Dosovitskiy_2021_ViT} in recent years, research on learning a single model for images and videos has emerged\cite{Fan_2022_SIFAR,Girdhar_CVPR2022_Omnivore,Likhosherstov_arXiv2021_PolyViT,Girdhar_arXiv2022_OmniMAE}. 
Although many CNN-based image and action recognition models have been proposed, most of them were developed separately. 
The reason for this is that there is a difference between images and videos in terms of time axis. 
An image is considered a moving image with one frame, and all information is contained within a single frame.
On the other hand, a video has more than two frames, and information is allocated to each frame, so it is necessary to consider which frame contains the most important information for learning. 
Although a action recognition model using a single RGB frame in a video was also proposed\cite{Wang_ECCV2016_TSN}, various innovations were proposed for handling temporal information in video recognition because it is important to model the temporal information\cite{Tran_2018CVPR_R(2+1)D,Wang_2018CVPR_NonLocal}.  
In this research stream, simultaneous learning of still images was not considered. 
However, as Transformer\cite{Vaswani_arXiv2017_transformer} became popular and ViT, an image recognition model, became successful, action recognition models based on ViT were proposed one after another\cite{Selva_ArXiv2022_Video_Trans_Survey}. 
ViT divides an image into patches and applies Transformer by considering the patches as tokens, while the ViT-based action recognition model divides a video into patches.
This structure allows the self-attention mechanism to play the role of acquiring temporal information and simplifies the design of the model by providing both images and videos in exactly the same way as inputs to the Transformer. 
The problem here is computational cost. The computational cost of ViT's self-attention mechanism is $O(N^2)$, where $N$ is the number of input patches.
The computational cost increases with increasing the number of patches as the video length increases, and conversely, the resolution in the time direction drops when the number of patches is fixed. Although some countermeasures have been proposed\cite{Bertasius_ICML2021_TimeSformer,Bulat_NeurIPS2021_X-ViT}, they are not suitable for handling images and videos simultaneously. In this study, we propose an efficient and computationally inexpensive model for simultaneous learning of images and videos.
The proposed method shown in Fig\ref{fig:proposed model overview} applies a two-dimensional image recognition model (ViT) to each frame, which is a simple method used as a baseline in action recognition\cite{Zhang_ACMMM2021_TokenShift}.
When recognizing images, ViT is applied, and when recognizing moving images, the output of ViT for each frame is aggregated by late fusion\cite{Karpathy_2014_CVPR}.
This structure enables simultaneous learning of images and videos using ViT without increasing the computational complexity.
However, because temporal information must be modeled, a method using temporal feature shift\cite{Hashiguchi_2022_ACCVW_MSCA,Lin_2019ICCV_TSM,Zhang_ACMMM2021_TokenShift} is applied.
In addition, to absorb the domain difference between images and videos, we apply multi-domain and multi-dataset learning methods\cite{Li_2019_CVPR,Omi_IEICE-ED2022_MDL}.

The contributions of this study are as follows

\begin{itemize}
    \item We propose a computationally inexpensive simultaneous learning model for images and videos using ViT.The proposed method learns a ViT model for a single image, applies ViT to the image as-is, and applies and aggregates ViT to the video frame by frame.
    \item We apply temporal feature shifting for simultaneous learning of images and videos. This is the first study in which a shifting method proposed for action recognition is used for simultaneous learning of images and videos.
    \item We propose a method to apply a multi-domain learning method to absorb the domain differences between images and videos.
    \item Evaluate performance on multiple image and video domains using multiple image and action recognition datasets.
\end{itemize}


\begin{figure}
\centering

\begin{minipage}[t]{0.6\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/method/method_image.pdf}
\subcaption{}
\end{minipage}

\vspace{2em}

\begin{minipage}[t]{0.8\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/method/method_video.pdf}
\subcaption{}
\end{minipage}

\caption{Schematic diagram of the proposed model based on ViT.
(a) When one image is entered．
(b) When a video clip consisting of $T$ frames is input.
}
\label{fig:proposed model overview}
\end{figure}

\section{related works}


\subsection{Image and Action recognition}

Since the emergence of ImageNet \cite{Deng_CVPR2009_ImageNet}, many methods using convolutional neural networks (CNN) have been proposed in the field of image recognition\cite{He_2016_CVPR,Alex_NeurIPS2012_AlexNet,Simonyan_arXiv2014_VGG,Szegedy_arXiv2014_GoogLeNet}, and recently, many models based on the Vision Transformer (ViT) \cite{Dosovitskiy_2021_ViT}, which is based on the Transformer\cite{Vaswani_arXiv2017_transformer}, have been proposed\cite{Liu_2021_ICCV,Zhang_ACMMM2021_TokenShift}.
With the development of image recognition models, there has also been a lot of research on action recognition, and many methods based on 3D CNN\cite{Joao_CVPR2017_I3D,Feichtenhofer_CVPR2020_x3d,Feichtenhofer_ICCV2019_SlowFast,Hara_CVPR2018_3DResNet,Du_ICCV2015_C3D} and ViT\cite{Arnab_ICCV2021_ViVit,Bertasius_ICML2021_TimeSformer,Neimark_2021_ICCVW_VideoTransformerNetwork,Sharir_arxiv2021_STAM,Zhang_ACMMM2021_TokenShift} have been proposed.
 Early studies proposed methods such as Two-Stream Network\cite{Karen_NeurIPS2014_TwoStream} using a single frame of video and optical flow, and Temporal Segment Network (TSN)\cite{Wang_ECCV2016_TSN} that applies a 2D CNN to multiple video segments. However, late fusion\cite{Karpathy_2014_CVPR}, which applies a 2D CNN to each frame and aggregates it in the temporal direction, is simple and is often used as a baseline method for comparison. However, late fusion alone is limited in its ability to model in the temporal direction, so the Temporal Shit Module (TSM)\cite{Lin_2019ICCV_TSM}, which exchanges intermediate layer features back and forth in time, has also been proposed.


\subsection{Simultaneous image and video learning}

Thus, image recognition models and action recognition models have been studied separately, but several attempts have been made to identify both images and videos with a single model.
UniDual\cite{Wang_arXiv2019_UniDual} and Omnisorce\cite{Duan_arXiv2020_OmniSource} are methods that unify the use of 3D CNN models such as SlowFast \cite{Feichtenhofer_ICCV2019_SlowFast} and R(2+1)D \cite{Tran_2018CVPR_R(2+1)D} by replicating a still image in the temporal direction and converting it to a 3D volume.
Unlike CNN, ViT uses patch segmentation (tokenizer), which makes it easier to handle different modes of data in a unified manner. Using this method, PolyVit \cite{Likhosherstov_arXiv2021_PolyViT} simultaneously learns images, videos, and audio, Omnivore \cite{Girdhar_CVPR2022_Omnivore} simultaneously learns images, videos, and 3D data, and OmniMAE \cite{Girdhar_arXiv2022_OmniMAE} pre-trains images and videos by using patch masks.

The problem with these methods is that they are computationally expensive. The method of converting a still image to a 3D volume\cite{Duan_arXiv2020_OmniSource,Wang_arXiv2019_UniDual} incurs unnecessary computational costs. The computational complexity of the self-attention mechanism of the ViT-based method\cite{Girdhar_CVPR2022_Omnivore,Likhosherstov_arXiv2021_PolyViT,Girdhar_arXiv2022_OmniMAE} is $O(N^2)$, and the longer the movie is, the larger the number of input patches $N$ becomes, which increases the computational cost.

On the other hand, in this study, ViT is applied to video frame by frame and aggregated by late fusion. The same process can be applied to still images by considering them as moving images with frame number 1. Therefore, the increase in computational cost is linearly proportional to the number of frames, even if the number of frames in the video increases.


\section{method}

In this section, we describe a more efficient simultaneous image and video learning model. The Vision Transformer (ViT) \cite{Dosovitskiy_2021_ViT} is used as the base model. However, ViT cannot handle inputs of different modes simultaneously if used as is. Therefore, in order to treat inputs with different modes in the same way, the inputs are transformed in advance. In addition, multiple heads are prepared for training on multiple datasets.


\subsection{ViT for Image}


Here is a brief description of the original ViT (for images) used in the base model. Let $x \in \R^{3 \times H \times W}$ be the input image, where $H$ and $W$ are the height and width of the image. The input image is first divided into $P \times P$ pixel patches by the tokenizer and transformed into a tensor $\hat{x} = [x_0^1, \ldots, x_0^N] \in \R^{N \times d}$ of patch rows. where $x_0^i \in \R^{d}$ is the $i$-th patch, $N = \frac{HW}{P^2}$ is the number of patches, and $d = 3 P^2$ is the patch dimension. The input patch $x_0^i$ is transformed by a linear transformation using the $D$-dimensional embedding matrix E and the addition of the position embedding $E_\mathrm{pos}$ as follows.

\begin{align}
    z_0 &= [c_0, x_0^1 E, x_0^2 E, \ldots, x_0^N E] + E_\mathrm{pos}
\end{align}


where $c_0 \in \R^{D}$ is a class token. This patch embedding $z_0 \in \R^{(N+1) \times D}$ is input to the first encoder block $M^\ell$ of the transformer.
Let $z_\ell$ be the input to the $\ell$-th block $M^\ell$ and $z_\ell$ be the output, the processing in the block can be expressed as follows.




\begin{align}
    z'_\ell &= \mathrm{MSA}(\mathrm{LN}(z_{\ell - 1})) + z_{\ell - 1}
    \\
    z_\ell &= \mathrm{MLP}(\mathrm{LN}(z'_\ell)) + z'_\ell,
\end{align}

where LN is layer normalization, MSA is multi-head self-attention, and MLP is the multilayer perceptron. This is denoted as follows.


\begin{align}
    z_{\ell} &= M^\ell (z_{\ell - 1})
\end{align}

then, The output $z_L$ of ViT consisting of $L$ blocks is able to denote as follows.

\begin{align}
    z_L = (M^L \circ M^{L-1} \circ \cdots M^1 \circ M^0) (x)
    \in \R^{(N+1) \times D}
\end{align}

Note that $\circ$ is the function synthesis and $M^0$ is the tokenizer. The class prediction is obtained by applying the head $M^h$, which consists of a linear layer and softmax.

\begin{align}
    \hat{y} &= M^h(z_L)
\end{align}


However, usually only the part of $z_L$ corresponding to the class token is used. Let $(n,d)$ elements of $z_\ell$ be denoted by $z_{\ell, n, d}$ and the elements of the part $\tilde{z}_\ell \in \R^D$ corresponding to the class token by $\tilde{z}_{\ell, d}$.

\begin{align}
    \tilde{z}_{\ell, d} &= z_{\ell, 0, d}
\end{align}
regarding
\begin{align}
    \hat{y} &= M^h(\tilde{z}_L) \in [0, 1]^C
\end{align}

where $C$ is the number of categories.


\subsection{ViT for frame-by-frame video}

In order to apply ViT\cite{Hashiguchi_2022_ACCVW_MSCA,Zhang_ACMMM2021_TokenShift} for images frame by frame, the above formulation is modified.  Let $x \in \R^{T \times 3 \times H \times W}$ be the input video clip. where $T$ is the number of frames in the video clip. Each frame is transformed into $N$ patches of $P \times P$ pixels $\hat{x} = [x_0^1, \ldots, x_0^N] \in \R^{T \times N \times d}$ by tokenizer. where $x_0^i \in \R^{T \times d}$ is the $i$th patch in the frame.  The patch embedding is the same as in the case of an image as follows.]


\begin{align}
    z_0 &= [c_0, x_0^1 E, x_0^2 E, \ldots, x_0^N E] + E_\mathrm{pos}
\end{align}


However, the dimension of the class token is $c_0 \in \R^{T \times D}$ and the dimension of the patch embedding is $z_0 \in \R^{T \times (N+1) \times D}$.  The output $z_L$ obtained by inputting this to ViT consisting of $L$ blocks $M^{\ell}$ is as follows.

\begin{align}
    z_L = (M^L \circ M^{L-1} \cdots M^1 \circ M^0) (x)
    \in \R^{T \times (N+1) \times D}
\end{align}


There are many possible ways to aggregate the output for $T$ frames\cite{Sharir_arxiv2021_STAM}, but in this study, we use the simplest method, temporal average pooling\cite{Hashiguchi_2022_ACCVW_MSCA,Zhang_ACMMM2021_TokenShift}. Let $(t,n,d)$ elements of $z_\ell$ be denoted by $z_{\ell,t, n, d}$ and $\tilde{z}_\ell \in \R^{T \times D}$ corresponding to the class token be denoted by $\tilde{z}_{\ell, t, d}$, the class token part:

\begin{align}
    \tilde{z}_{\ell, t, d} &= z_{\ell, t, 0, d}
\end{align}

The average pooling for $\tilde{z}_{\ell, t, d}$ is

\begin{align}
    \bar{z}_{\ell, d} &= \frac{1}{T} \sum_t^T \tilde{z}_{\ell, t, d}
\end{align}

And the prediction obtained by applying the head is

\begin{align}
    \hat{y} &= M^h(\bar{z}_L) \in [0, 1]^C
\end{align}


\subsection{Proposed Model}

The aforementioned ViT for images and for video can be handled in a unified manner by processing each batch. In general, the input to the model is a batch $x \in \R^{B \times 3 \times H \times W}$ of batch size $B$, which is a bundle of images for each $B$, and the output $\hat{y} \in [0, 1]^{B \times C}$ to it is also in batch units. In other words, the input/output of the above ViT block $M_\ell$ is also $z_\ell \in \R^{B \times (N+1) \times D}$. Therefore, the block does not need to distinguish whether the input is a video frame or a batch of images.  Therefore, the same ViT block is applied to image and video by changing the treatment of input and output as follows.


\subsubsection*{Image input}


Take a batch of images $x \in \mathbb{R}^{B \times 3 \times H \times W}$ as input. The output of the $L$-th block is $z_L \in \R^{B \times (N+1) \times D}$, and the class token part $\tilde{z}_L \in \R^{B \times D}$ identified by the head is $\hat{y} \in [0, 1]^{B \times C}$. The output identified by the head is $\hat{y} \R^{B \times D}$.  This is the same process used in ViT for image processing when handling batches.


\subsubsection*{Video input}

Take a batch of video clips $x \in \mathbb{R}^{B \times T \times 3 \times H \times W}$ as input. To input this 5D tensor to ViT, the frame dimension is expanded to the batch dimension and transformed into a 4D tensor $x' \in \mathbb{R}^{BT \times 3 \times H \times W}$.    The output of the $L$-th block is $z_L \in \mathbb{R}^{BT \times (N+1) \times D}$, which is first transformed into $z'_L \in \mathbb{R}^{BT \times T \times (N+1) \times D}$. Then, the class token part $\tilde{z}'_L \in \mathbb{R}^{B \times T \times D}$ is extracted and average pooling is applied to obtain $\bar{z}'_L \in \mathbb{R}^{B \times D}$. The output identified by the head is $\hat{y} \in [0, 1]^{B \times C}$.

\subsection*{Challenges in Implementation}

As mentioned above, there are many considerations when implementing a model that takes images and video as input.

\subsubsection*{Pre-trained model weights}

When the dataset size is small, it is common practice to use weights from models pre-trained on large datasets as initial values.
For image recognition, it is standard to use weights pre-trained on ImageNet-1k or 21k, and for action recognition, weights pre-trained on Kinetics-400 are often used.
However, in this study, the same model is used to discriminate images and videos, so the prior weights need to be effective for both images and videos. Therefore, it is necessary to investigate which dataset, image or video, is more effective for pre-training weights.


In our experiments, we compare the performance of ViT with weights pre-trained on ImageNet-21k\footnote{\url{https://github.com/lukemelas/PyTorch-Pretrained-ViT}} and with weights pre-trained on Kinetics-400 for a model that applies ViT at each frame\footnote{\url{https://github.com/VideoNetworks/TokShift-Transformer}}.


\subsubsection*{Hyperparameter selection}

Since the optimal hyperparameters differ for each dataset, different optimization methods, different learning rates, and different values of weight decay are often used for each dataset\cite{Likhosherstov_arXiv2021_PolyViT}.
However, when using the same model for images and video, the same hyperparameters are not always appropriate, even though they are different modalities.
Furthermore, when dealing with multiple image and video datasets, it is not realistic to search for the appropriate hyperparameters for all datasets, and even if the optimal hyperparameters are found for each dataset, they may not be effective when training on multiple datasets.   Therefore, we compare the following hyperparameter settings in our experiments.


\begin{itemize}
\item all：Unify settings for all datasets. Even if there are multiple image datasets or multiple video datasets, use the same settings for all of them.

\item domain：The settings are standardized for images and videos, respectively. Multiple image datasets use common settings among them, and multiple video datasets use common settings among them. However, images and videos do not necessarily share the same settings.

\item each：Use separate settings for each dataset. Use separate settings for each dataset.
Separate experiments are conducted to determine the value, and the appropriate value is used when each dataset is trained separately.
\end{itemize}


\begin{figure}
\centering

\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/all.pdf}
\subcaption{}
\end{minipage}
\hfil
\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/domain.pdf}
\subcaption{}
\end{minipage}
\hfil
\begin{minipage}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/optimizer/each.pdf}
\subcaption{}
\end{minipage}

\caption{Various settings for optimizer methods．
(a) all：To unify all data sets．
(b) domain：When unified with image and video data sets．
(c) each：To set for each data set．
}
\label{fig:hyperparameter selection}
\end{figure}



\subsubsection*{Modeling of temporal information}


The proposed method uses frame-by-frame ViT to extract features, and applies average pooling in the temporal direction to predict each video frame.
However, the frame-by-frame ViT is not sufficient to model the temporal information of the video.
Therefore, we introduce a method that can handle temporal information while maintaining this structure.
Specifically, we use TokenShift\cite{Zhang_ACMMM2021_TokenShift} and MSCA\cite{Hashiguchi_2022_ACCVW_MSCA}, which introduce TSM\cite{Lin_2019ICCV_TSM} to ViT.



\begin{figure}[t]

    \centering
    
    
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/ViT.pdf}\\
    \subcaption{}
    \label{fig:ViT_block}
    \end{minipage}
    \hfil
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/tokenshift.pdf}
    \subcaption{}
    \label{fig:tokenshift_block}
    \end{minipage}
    \hfil
    \begin{minipage}{.25\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/model/MSCA.pdf}
    \subcaption{}
    \label{fig:MCSA_block}
    \end{minipage}

    
    \caption{
    Encoder block for each model．
    (a) ViT \cite{Dosovitskiy_2021_ViT}，
    (b) TokenShift \cite{Zhang_ACMMM2021_TokenShift}，
    (c) MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}．
    }
    \label{Fig:overview}

\end{figure}


In these methods, for the time dimension $t$ of $z_{\ell, t, n, d}$ in the $\ell$-th block $M^\ell$,　it is peformed the feature shift\cite{Zhang_ACMMM2021_TokenShift} or the attention shift\cite{Hashiguchi_2022_ACCVW_MSCA}. In this method, one block of information is propagated in the time direction for one time period. Therefore, if the input video clip length is $T$ frames, it is possible to interact with temporal information for the whole time by setting the number of blocks to $L \ge T$\cite{Hashiguchi_2022_ACCVW_MSCA}.


\subsubsection*{Weighting of loss functions}

Different data sets generally have different numbers of categories.
Therefore, it is common to use a multi-head structure in which a head is provided for each dataset\cite{Omi_IEICE-ED2022_MDL}.
Let $\mathcal{D}_i$ be the $i$-th dataset, $C_i$ the number of categories, $M^h_i$ the head, and $\mathcal{L}_i()$ the loss function associated with this head.


In this method, the input batch to the model is sampled from a single dataset. That is, if $(x, y)$ is a pair of a batch of data and its teacher label, the loss function is as follows\cite{Omi_IEICE-ED2022_MDL}.


\begin{align}
    \mathcal{L}
    &=
    E_{\mathcal{D}_i \sim \mathcal{D}}
    E_{ (x, y) \sim \mathcal{D}_i}
    \left[ \mathcal{L}_i( \hat{y}, y ) \right]
\end{align}


where $\mathcal{D} = \{ \mathcal{D}_1, \ldots, \mathcal{D}_{D_N} \}$ is a set of $D_N$ data sets.

Although there are many possible ways to sample a dataset, it has been reported that the method of obtaining samples in proportion to the dataset size performs well\cite{Likhosherstov_arXiv2021_PolyViT}.
In this study, instead of sampling, we consider approximating the loss function by a weighted sum of the loss function for each dataset and the empirical loss per batch, as follows.


\begin{align}
    \mathcal{L}
    &=
    \sum_{i=1}^{D_N}
    w_i
    \mathcal{L}_i \\
    \mathcal{L}_i
    &=
    \frac{1}{S_i}
    \sum_{b=1}^{S_i}
    \mathcal{L}_i( \hat{y}_b, y_b )   
\end{align}


where $S_i$ is the number of batches that can be sampled from dataset $i$ (the number of data is multiplied by the batch size) and $\hat{y}_b, y_b$ are the predicted and true value labels for batch $b$. The actual per-batch update is a gradient calculation using the following, which incorporates the weights into the per-batch loss.

\begin{align}
    w_i \mathcal{L}_i( \hat{y}_b, y_b )   
\end{align}

Here, we use two methods proposed for multi-task learning\cite{Crawshaw_arXiv2020_Multi-Task_survey,Vandenhende_TPAMI2022_Multi-Task_survey} as weights $w_i$.
In multi-task learning, the learning speed differs for each task, so it is necessary to control the learning speed by weights.
In this study, video have multiple frames, so the learning convergence is considered to be slower than that of images.
Therefore, we introduce weights that depend on the learning rate, instead of simple fixed weights that depend on the dataset size, to mitigate the difference in learning rate for each dataset.


\begin{description}

\item[Dynamic Task Prioritization (DTP)
    \cite{Guo_2018ECCV_Dynamic_Task_Prioritization}]
The weights $w_i$ are defined according to the learning degree of the dataset by the following equation.
\begin{align}
    w_i(t) = - (1 - \kappa_i(t))^{\gamma_i} \log{\kappa_i(t)}
\end{align}
where $\kappa_i(t)$ is the performance index at the $t$th iteration for dataset $i$, $\gamma_i$ is the weight for loss (focusing parameter)\cite{Lin_2017_ICCV_focal_loss}，
$t$ is the number of iterations (number of batches).


\item[Dynamic Weight Averaging (DWA)
      \cite{Liu_2019CVPR_DWA_Dynamic_Weight_Averaging}]
Define the weight $w_i$ according to the degree of decrease in the most recent loss function value as
\begin{align}
    w_{i}(t) &= \frac{N\exp(r_i(t-1)/T)}{\sum_{n=1}^{D_N}{\exp(r_n(t-1)/T)}} \\
    r_i(t-1) &= \frac{\mathcal{L}_i(t-1)}{\mathcal{L}_i(t-2)}
\end{align}
where $D_N$ is the number of data sets, $T$ is the temperature parameter, $\mathcal{L}_i(t)$ is the loss value at the $t$th iteration for data set $i$, and $t$ is the number of iterations (batches).
\end{description}


In multi-task learning\cite{Crawshaw_arXiv2020_Multi-Task_survey,Vandenhende_TPAMI2022_Multi-Task_survey}, multiple loss functions are computed for a single sample, whereas in multi-domain learning\cite{Omi_IEICE-ED2022_MDL} and multi-dataset learning\cite{Liang_NeurIPS2022_Multi-Dataset}, only one loss function is computed for a given sample.


%%%%%%%%%%%%%%%%%% 事前重みの選定の実験 %%%%%%%%%%%%%%%%%%%

\begin{figure*}

    \centering

    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/TinyI.pdf}
        \subcaption{Tiny-ImageNet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/CIFAR100.pdf}
        \subcaption{CIFAR100}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/UCF101.pdf}
        \subcaption{UCF101}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/pretrain/K200.pdf}
        \subcaption{mini-Kinetics}
    \end{minipage}

    \caption{各データセット個別の学習における，
    ImageNet-21k（I21k）とKinetics400（K400）での事前学習済み重みを用いた場合の性能の比較
    }
    \label{fig:pretrain}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{experiments}


To evaluate the proposed method, experiments were conducted on several datasets to compare the performance of various settings.


\subsection{Experimental Settings}


\subsubsection*{Datasets}

In our experiments, we use the following two types of image datasets and two types of video datasets. That is, the two domains are images and videos, and the total number of datasets is $D_N=4$.

\begin{itemize}

\item Tiny-ImageNet \cite{Tiny_ImageNet_kaggle2018}：
Image dataset consisting of 100,000 training images and 10,000 validation images. Each training image is a $64$ pixel image extracted from 200 ImageNet classes (500 images per class).

\item CIFAR-100 \cite{Krizhevsky_TR2009_CIFAR10-100}：
An image dataset consisting of 50,000 training images and 10,000 validation images. The number of categories is 100 and the image size is $32 \times 32$.

\item Mini-Kinetics (Kinetics-200) \cite{Xie_2018ECCV_S3D_Kinetics200}：
Action recognition dataset consisting of 78246 training videos and 5000 validation videos. Each video is extracted from 200 classes of Kinetics-400 (about 400 videos for each class).


\item UCF101 \cite{Soomro_arXiv2012_UCF101}：
A 101-class action recognition dataset consisting of 9537 training videos and 3783 validation videos.

\end{itemize}

For both datasets, the top-1 (val top-1) of the validation set is used to evaluate the performance.
The top-1 (val top-1) of the validation set is used to evaluate performance.



\subsubsection*{Model}

In our experiments, we use Vision Transformer \cite{Dosovitskiy_2021_ViT} as the base model for the proposed method, TokenShift\cite{Zhang_ACMMM2021_TokenShift} and MSCA \cite{Hashiguchi_2022_ACCVW_MSCA}.
Since a head exists for each dataset, each model has four heads.

\subsubsection*{Learning Samples}

For an image dataset, we randomly crop one image to $[0.08, 1.0]$ times the size of the original image, randomly determine the aspect ratio in the range $[\frac{3}{4}, \frac{4}{3}]$, and resize it to $224 \times 224$ pixels Resize the image to $224$ pixels. After that, the image is flipped horizontally with a probability of $1/2$.   For the video dataset, a clip is created by extracting consecutive frames corresponding to a specified number of seconds (clip time) from a video and sampling 16 frames uniformly in the time direction from the extracted frames. The sampling rate varies depending on the dataset (and video), but in the experiment, the clip time was fixed at approximately 2.67 seconds. The short edge of the extracted frame is randomly determined within $[224, 320]$ pixels, and resized while maintaining the aspect ratio. Then $224 \times 224$ pixels at random locations are cropped and flipped horizontally with a probability of $1/2$.

\subsubsection*{Batch sampling}

When training multiple datasets simultaneously, it is necessary to consider the order in which to sample batches from each dataset and the ratio of sampling batches for each dataset\cite{Likhosherstov_arXiv2021_PolyViT}.
In this method\cite{Omi_IEICE-ED2022_MDL}, batches are sampled and parameters are updated in the same way as in the previous method.


\begin{itemize}
\item 

The order of dataset sampling is fixed: Tiny-ImageNet, CIFAR100, UCF101, and mini-Kinetics, in that order.

\item


For each dataset, the batch size is fixed to 6, sampled one batch at a time. Thus, a mini-batch of an image dataset consists of 6 images, and a mini-batch of a video dataset consists of 96 frames, since each of the 6 videos consists of 16 frames.

\end{itemize}


A mini-batch is sampled from each dataset, the gradient is computed, and the parameters are updated. This is one iteration.


\subsection{Selection of pre-trained model weights}


First, we compare the performance of the weights of ViT, the base model, on each dataset individually, using the weights pre-trained on ImageNet-21k and using the weights pre-trained on Kinetics400.
The number of training iterations was fixed at 50000.
The optimization method was SGD, and the learning rate was set to 1e-4 for the image dataset and 1e-3 for the video dataset. The default values of other parameters are shown in Tab\ref{Tab:default}.


 The results are shown in Fig\ref{fig:pretrain}. For the image datasets Tiny-ImageNet and CIFAR100, the performance of Kinetics400 weights is higher in the early stages of learning, although there is no difference between Kinetics400 and ImageNet-21k weights in the end. On the other hand, for the video datasets UCF101 and mini-Kinetics, the Kinetics400 weights consistently outperform the Kinetics21k weights. From the above, the weights pre-trained by Kinetics400 will be used in the following experiments.



 %%%%%%%%%%% 最適化手法のデフォルト値 %%%%%%%%%%%
\begin{table}[t]
  \centering
  \caption{Default values for each optimization method}
  \label{Tab:default}

\scalebox{0.8}{
  \begin{tabular}{c|cccc}
     & weight decay & momentum & $ \beta_1 $ & $ \beta_2 $ \\
     \hline
     SGD & 5e-5 & 0.9 & -- & -- \\
     Adam & 5e-5 & -- & 0.9 & 0.999 \\
     AdamW & 5e-5 & -- & 0.9 & 0.999 
  \end{tabular}
}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%% optimizer選定の事前実験の性能図 %%%%%%%%%%%%%%%%%
\begin{figure*}

    \centering
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/TinyI.pdf}
        \subcaption{Tiny-ImageNet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/CIFAR100.pdf}
        \subcaption{CIFAR100}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/UCF101.pdf}
        \subcaption{UCF101}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/K200.pdf}
        \subcaption{mini-Kinetics}
    \end{minipage}
    
    \caption{Comparison of the performance of 9 optimization methods and learning rates for learning each dataset individually
    }
    \label{fig:dataset_opt_acc}
\end{figure*}



\begin{table*}[t]

  \centering
  \caption{Comparison of the performance of varying the optimization and learning rate for individual training on each dataset.}
  \label{Tab:dataset_opt_acc}

 
\begin{tabular}{cc|cccccccc}
 \multicolumn{2}{c}{} &  \multicolumn{2}{c}{Tiny-ImageNet} & \multicolumn{2}{c}{CIFAR100} &  \multicolumn{2}{c}{UCF101} &  \multicolumn{2}{c}{mini-Kinetics} \\
optimizer & lr & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ 
\hline
Adam & 1e-3 & \phantom{0}6.95 & 21.39 & 15.19 & 41.27 & 16.8 & 43.41 & \phantom{0}2.66 & 88.54 \\
     & 1e-4 & 68.11 & 88.05 & 80.94 & 96.80 & 76.19 & 93.07 & 24.12 & 53.64\\
     & 1e-5 & \textbf{81.90} & 94.30 & 88.89 & 98.81 & 87.43 & 98.04 & \textbf{68.26} & 88.68 \\
\hline
AdamW & 1e-3 & \phantom{0}0.50 & \phantom{0}2.50 & \phantom{0}9.35 & 29.70 & 0.85 & \phantom{0}4.81 & \phantom{0}0.50 & \phantom{0}2.50 \\
      & 1e-4 & 70.33 & 89.54 & 81.66 & 97.10 & 79.42 & 93.60 & 58.58 & 82.98 \\
      & 1e-5 & 81.27 & 94.36 & \textbf{89.19} & 98.77 & 88.15 & 97.86 & 68.20 & 88.40 \\
\hline
SGD & 1e-3 & 81.60 & 94.85 & 87.90 & 98.56 & \textbf{90.50} & 98.81 & 66.82 & 87.96 \\
    & 1e-4 & 79.78 & 93.53 & 88.04 & 98.68 & 87.59 & 98.62 & 66.90 & 88.06\\
    & 1e-5 & 14.78 & 33.80 & 57.31 & 83.68 & 62.91 & 88.54 & 16.56 & 36.06 \\

\end{tabular}


\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{How to set hyperparameters}


Next, we compare the performance of the optimization method and hyperparameters for simultaneous training of multiple datasets when they are unified for all datasets (all), for images and videos (domain), and for each dataset individually (each).
In this experiment, we compare the performance of three optimization methods (SGD, Adam\cite{Kingma_ICLR2015_Adam}, and AdamW \cite{Loshchilov_ICLR2019_AdamW}) and three hyperparameters (1e-3, 1e-4, and 1e-5) limited only to the learning rate, for a total of nine different settings.   However, since it is not realistic to compare all combinations of settings, we first determined the settings that were effective for individual training on each dataset through preliminary experiments, and then determined the all, domain, and each settings based on these results.

\subsubsection*{preliminary experiment}


The results of the individual training for each dataset are shown in Fig\ref{fig:dataset_opt_acc} and Tab\ref{Tab:dataset_opt_acc}, using the nine settings described above.
The number of training iterations was set to 50000, and other settings were as described above.



\begin{itemize}

\item 
The combination of (Adam, 1e-3), (AdamW, 1e-3), and (SGD, 1e-5) does not perform well on any dataset, while (Adam, 1e-5), (AdamW, 1e-5), (SGD, 1e-3), and (SGD, 1e-4) for all datasets. The best performing combinations for each dataset are (Adam, 1e-5) for Tiny-ImageNet, (AdamW, 1e-5) for CIFAR100, (SGD, 1e-3) for UCF101, and (Adam, 1e-5) for mini-Kinetics. The following is the setting of EACH.

\item
Comparing image and video datasets, (Adam, 1e-5) performs relatively well on Tiny-ImageNet and CIFAR100, and (AdamW, 1e-5) performs relatively well on UCF101 and mini-Kinetics, both of which are video datasets. (AdamW, 1e-5) for the video datasets UCF101 and mini-Kinetics. Therefore, these are used as the domain settings.

\item
For the all setting, we adopt (AdamW, 1e-5), which is valid on average for all data sets.
\end{itemize}


Tab\ref{Tab:optimizer} below shows the settings for the three cases selected from the above.


\begin{table*}[t]
  \centering
  \caption{Optimization methods and learning rates used for all, domain, and each case.}
  \label{Tab:optimizer}

  \begin{tabular}{c|cccccccc}
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Tiny-ImageNet} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{UCF101} & \multicolumn{2}{c}{mini-Kinetics} \\
    setting & optimizer & lr & optimizer & lr & optimizer & lr & optimizer & lr \\
    \hline
    all     & AdamW & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 \\
    domain  & Adam & 1e-5 & Adam & 1e-5 & AdamW & 1e-5 & AdamW & 1e-5 \\
    each    & Adam & 1e-5 & AdamW & 1e-5 & SGD & 1e-3 & Adam & 1e-5 \\
    
  \end{tabular}
\end{table*}


\subsubsection*{Learning}


Using the settings selected in the preliminary experiment described above, we compare the all, domain, and each cases. The number of training iterations is set to 100000 and the batch size to 4. The weights of the ViT-based model are the ones pre-trained with Kinetics400.


The results are shown in Fig\ref{fig:optimizer}.
In the all case(figure\ref{fig:optimizer all}), all datasets were successfully trained in the end. In contrast,
in the domain(figure\ref{fig:optimizer domain}) and each(figure\ref{fig:optimizer each}) cases, some datasets fail to learn. This suggests that the appropriate hyperparameter settings are different when training multiple datasets simultaneously than when training individual datasets. Although learning may be successful in the domain and each case with other values, we use the all setting in the subsequent experiments in this study.



%%%%%%%%%%%%%%%% 最適化手法の選定の性能図，表 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/all_graph.pdf}
        \subcaption{all}
        \label{fig:optimizer all}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/domain_graph.pdf}
        \subcaption{domain}
        \label{fig:optimizer domain}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/each_graph.pdf}
        \subcaption{each}
        \label{fig:optimizer each}
    \end{minipage}

    \caption{
    Comparison of performance for different hyperparameter settings.
    }
    \label{fig:optimizer}
\end{figure*}



\begin{table*}[t]

  \centering
  \caption{Comparison of performance for different hyperparameter settings. average is a simple average of the performance for each dataset.}
  \label{tab:optimizer}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  setting & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
  
all    & 82.80 & 95.02 & 89.48 & 98.74 & 90.79 & 98.76 & 67.94 & 88.12 & 82.75 & 95.16 \\
domain & 80.78 & 94.05 & \phantom{0}5.86 & 26.68 & \phantom{0}7.75 & 20.29 & \phantom{0}1.44 & \phantom{0}6.80 & 23.96 & 36.96\\
each   & 76.60 & 92.81 & 84.85 & 97.84 & 83.84 & 96.27 & \phantom{0}5.10 & 15.34 & 62.60 & 75.57\\
\end{tabular}


\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Comparison of temporal information modeling}

Next, we compare the performance of a simple frame-by-frame ViT with that of using TokenShift \cite{Zhang_ACMMM2021_TokenShift} and MSCA \cite{Hashiguchi_2022_ACCVW_MSCA} to model temporal information.
All training settings are the same as in the all case selected in the previous section.

The results are shown in Figure\ref{fig:temporal models}.
It can be seen that the training is stable for all models, and there is no significant difference in performance.
Table\ref{tab:temporal models} shows the performance of Fig\ref{fig:temporal models}.
TokenShift outperforms the other two models on average, and all but Tiny-ImageNet perform better on individual datasets.
In particular, for the video dataset UCF101, there is a difference of about 1 percent. Based on the above, we will use TokenShift as the base model in the next experiment.


\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/optimizer/all_graph.pdf}
        \subcaption{ViT}
        \label{fig:temporal model ViT}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/tokenshift_result.pdf}
        \subcaption{TokenShift}
        \label{fig:temporal model TokenShift}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/MSCA_result.pdf}
        \subcaption{MSCA}
        \label{fig:temporal model MSCA}
    \end{minipage}

    \caption{
    Comparison of performance for different modeling of temporal information. The training setup is the same for all\ref{fig:optimizer all}. \subref{fig:temporal model ViT} is the same as in Fig.
    }
    \label{fig:temporal models}
\end{figure*}


\begin{table*}[t]

  \centering
  \caption{Comparison of performance for different modeling of temporal information. average is a simple average of the performance for each dataset.}
  \label{tab:temporal models}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
ViT        & 83.55 & 95.06 & 88.89 & 98.80 & 90.42 & 98.39 & 67.78 & 87.58 & 82.66 & 94.96 \\
TokenShift & 83.29 & 95.14 & 89.37 & 98.72 & 91.24 & 98.65 & 67.82 & 88.74 & 82.93 & 95.31 \\
MSCA       & 82.51 & 94.96 & 89.12 & 98.68 & 89.97 & 98.92 & 66.58 & 86.98 & 82.05 & 94.89 \\
\end{tabular}


\end{table*}


\subsection{Selection of loss weighting method}

Next, we compare the case without dynamic weighting for loss of multiple datasets ($w_i=1$), using DTP \cite{Guo_2018ECCV_Dynamic_Task_Prioritization}, and using DWA \cite{Liu_2019CVPR_DWA_Dynamic_Weight_Averaging}.

The number of training iterations is 100000 and the batch size is 4. The model is TokenShift, the prior weights are Kinetics400 pretrained, and the hyperparameters are the same as for all.
The DTP performance indicator $\kappa_i(t)$ is the average of the top-1 performance of each dataset on the training set over the last 500 iterations (only the updates on the corresponding dataset out of 2000 iterations for the entire dataset), and the focusing parameter is the same for all datasets with $\ gamma_i = 1$.
The temperature parameter of DWA was set to $T = 1$, and the loss $L(t)$ was the average of the loss for the last 500 iterations of the training set for each dataset (as above).

The results are shown in Fig\ref{Fig:loss_weighting}.
Fig\ref{Fig:loss_weighting} shows the trend of accuracy in each case, Fig\ref{fig:static loss weight} is the same as TokenShift(Fig\ref{fig:temporal model TokenShift}) in the previous section.


There is no significant difference in the learning trend between the cases with(Fig\ref{fig:DWA loss weight}, Fig\ref{fig:DTP loss weight}) and without DWA and DTP(Fig\ref{fig:static loss weight}), and the learning is stable.
Tab\ref{tab:loss_weighting} shows the results at the end of the training of Fig\ref{Fig:loss_weighting}.
The average performance with DTP was lower than that without weighting, and the performance with DWA was the best.


%%%%%%%%%%%%%%%%%%%%% lossの重みづけの性能図，表 %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]

    \centering

    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/model/tokenshift_result.pdf}
        \subcaption{static weight}
        \label{fig:static loss weight}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/loss/dwa.pdf}
        \subcaption{DWA}
        \label{fig:DWA loss weight}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/loss/task_prio.pdf}
        \subcaption{DTP}
        \label{fig:DTP loss weight}
    \end{minipage}

    \caption{
    Comparison of performance for different loss weighting methods.     The model is TokenShift and the training setting is all. \subref{fig:DWA loss weight} is the same as in Fig\ref{fig:temporal model TokenShift}. 
    }
    \label{Fig:loss_weighting}
\end{figure*}




\begin{table*}[t]

  \centering
  \caption{Comparison of performance for different loss weighting methods. average is a simple average of the performance for each dataset.}
  \label{tab:loss_weighting}

 
\begin{tabular}{c|cccccccc|cc}
  & \multicolumn{2}{c}{Tiny-ImageNet} 
  & \multicolumn{2}{c}{CIFAR100}
  & \multicolumn{2}{c}{UCF101}
  & \multicolumn{2}{c}{mini-Kinetics}
  & \multicolumn{2}{c}{average} \\
  & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\ \hline
static  & 83.29 & 95.14 & 89.37 & 98.72 & 91.24 & 98.65 & 67.82 & 88.74 & 82.93 & 95.31 \\
DWA     & 83.76 & 95.41 & 89.40 & 98.83 & 90.82 & 98.73 & 68.44 & 88.12 & 83.11 & 95.27 \\
DTP     & 80.80 & 94.49 & 87.80 & 98.47 & 89.05 & 98.54 & 62.28 & 85.44 & 79.98 & 94.24 \\
\end{tabular}


\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{conclusion}

In this paper, we propose a model that can handle images and videos in the same model, and study its learning method. Future work includes the adoption of another model that handles the temporal information lost by frame segmentation of video, and the modification of simple late fusion by mean pooling in video identification.
